Wireless coverage prediction via parametric shortest paths

When deciding where to place access points in a wireless network, it is useful to model the signal propagation loss between a proposed antenna location and the areas it may cover. The indoor dominant path (IDP) model, introduced by W\"{o}lfle et al., is shown in the literature to have good validation and generalization error, is faster to compute than competing methods, and is used in commercial software such as WinProp, iBwave Design, and CellTrace. Previously, the algorithms known for computing it involved a worst-case exponential-time tree search, with pruning heuristics to speed it up. We prove that the IDP model can be reduced to a parametric shortest path computation on a graph derived from the walls in the floorplan. It therefore admits a quasipolynomial-time (i.e., $n^{O(\log n)}$) algorithm. We also give a practical approximation algorithm based on running a small constant number of shortest path computations. Its provable worst-case additive error (in dB) can be made arbitrarily small via appropriate choices of parameters, and is well below 1dB for reasonable choices. We evaluate our approximation algorithm empirically against the exact IDP model, and show that it consistently beats its theoretical worst-case bounds, solving the model exactly (i.e., no error) in the vast majority of cases.

==> apx_alg.tex <==
\section{Approximate the Pareto set}
\label{sec:apx-alg}

% Macros:
% The path table
\newcommand{\PathTable}[2]{\Pi_{#1}^{#2}}
% Error
\newcommand{\approxerr}{\delta}
\newcommand{\err}{\epsilon}
% number of nodes
\newcommand{\numNodes}{n}
% number of edges
\newcommand{\numEdges}{\dimm}
%
\newcommand{\Lmax}{L_{\max}}

In this section, we present another approximation algorithm by approximating the Pareto set.  The algorithm is described in Algorithm~\ref{alg:pareto}, which is based on \cite{DBLP:journals/mst/TsaggourisZ09}.  In Algorithm~\ref{alg:pareto}, for each vertex $v \in \nodes$ and $i \in
\{0,1,2,\dots,\numNodes-1\}$, we maintain a table of paths $\PathTable{v}{i}$.
%, where $N=\lceil \frac{n l_{\max}}{\delta} \rceil$.
Each entry $\Path=\PathTable{v}{i}(j)$ denotes the $s-v$ path with the least
distance among all the $s-v$ paths with at most $i$ edges and $\lceil
\loss(\Path)/\approxerr \rceil = j$.  The algorithm iteratively construct $\PathTable{v}{i}$ by extending paths with at most $i-1$ edges in $\cup_{u \in \nodes} \PathTable{u}{i-1}$.  Note that for any $v \in \nodes$ and $i \in \{0,1,2,\dots \numNodes-1\}$, the number of paths in $\PathTable{v}{i}$ is upper-bounded by $\lceil \frac{\Lmax}{\approxerr} \rceil + 1$, where $\Lmax = \max_{\Path \in \Paths} \loss(\Path)$ is the maximum loss among all feasible paths.

\begin{algorithm}
	\caption{Approximation algorithm based on approximating the Pareto set}
	\label{alg:pareto}
	\begin{algorithmic}[1]
		\STATE Initialize: Let $\PathTable{\src}{0}=\{ \src \}$ and $\PathTable{v}{0}=\emptyset$ for all $v\not=\src$.
		\FOR {$i=1,\dots,\numNodes-1$}
		\STATE Set $\PathTable{v}{i}=\PathTable{v}{i-1}$ for each $v \in \nodes$.
		\FOR {each node $v\in \nodes$}
		\FOR {each $\src-v$ path $\Path \in \PathTable{v}{i-1}$}
		\FOR {each edge $(v,u)\in \edges$}
		\STATE Set $P'=$ augmenting $P$ by adding $(v,u)$.
		\STATE Set $j=\lceil \loss(\Path)/\delta \rceil$.
		\IF {$\PathTable{u}{i}=\emptyset$ or $\dist(\Path')<\dist(\PathTable{u}{i})$}
		\STATE Set $\PathTable{u}{i}=\Path'$.
		\ENDIF
		\ENDFOR
		\ENDFOR
		\ENDFOR
		\ENDFOR
		\STATE Return $\argmax_{\Path \in \Pi_\dest^{n-1}} \obj(\Path)$%, \forall \dest \in \nodes$.
	\end{algorithmic}
\end{algorithm}

The correctness and the performance of Algorithm~\ref{alg:pareto} is presented in the following theorem.  The proof is deferred to the appendix due to space constraints.
\begin{thm}\label{thm:approx}
	If $\optpair$ is the distance-loss for the dominant path to
	destination $\dest$, then Algorithm~\ref{alg:pareto} returns an \st path with $\obj(\Path) \leq \obj \optpair + \err$ in $O\left(\numNodes^2 \numEdges \frac{\Lmax}{\err}\right)$ time.
	%Algorithm~\ref{alg:pareto} finds the $\err$-additive approximation solution for the dominant path problem in $O\left(\numNodes^2 \numEdges \frac{\Lmax}{\err}\right)$ time and	$O\left(\numNodes^2 \frac{\Lmax}{\err}\right)$ space.
\end{thm}



% These last lines are necessary for the proper operation of AuCTeX.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 
